Energy-based Modelling of the Feedback Control of Biomolecular Systems with Cyclic Flow Modulation

Energy-based modelling brings engineering insight to the understanding of biomolecular systems. It is shown how well-established control engineering concepts, such as loop-gain, arise from energy feedback loops and are therefore amenable to control engineering insight. In particular, a novel method is introduced to allow the transfer function based approach of classical linear control to be utilised in the analysis of feedback systems modelled by network thermodynamics and thus amalgamate energy-based modelling with control systems analysis. The approach is illustrated using a class of metabolic cycles with activation and inhibition leading the concept of Cyclic Flow Modulation.

==> BG-defs.tex <==
%% Referencing and indexing
%%\newcommand{\Index}[1]{\emph{#1}\index{\MakeLowercase{#1}}}
\newcommand{\Index}[1]{\emph{#1}\index{#1}}
\newcommand{\IndeX}[1]{\emph{#1}\index{#1}}
\newcommand{\Ref}[1]{\ref{#1}, p.\pageref{#1}}
\newcommand{\cref}[1]{Chapter~\Ref{#1}}
\newcommand{\aref}[1]{Appendix~\Ref{#1}}
\newcommand{\sref}[1]{\S~\Ref{#1}}
\newcommand{\fref}[1]{Figure~\Ref{#1}}
\newcommand{\eref}[1]{Equation~\eqref{#1}}
\newcommand{\nitem}[3]{\item[#1] #2 \sref{#3}\index{#1}}
\newcommand{\eoe}{$\bm{\Diamond}$} % End of example mark.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "book"
%%% End:

